Impact of Dust on Spectral Distortion Measurements of the Cosmic Microwave Background

Spectral distortions of the cosmic microwave background (CMB) are sensitive to energy injection by exotic physics in the early universe. The proposed Primordial Inflation Explorer (PIXIE) mission has the raw sensitivity to provide meaningful limits on new physics, but only if foreground emission can be adequately modeled. We quantify the impact of interstellar dust on Compton $y$ and $\mu$ measurements by considering a range of grain size distributions and compositions constrained by theoretical and observational priors (Zelko & Finkbeiner 2020). We find that PIXIE can marginalize over a modest number of dust parameters and still recover $y$ and $\mu$ estimates, though with increased uncertainty. As more foreground components are included (synchrotron, free-free), the estimates of $y$ degrade, and measurement of $\mu$ in the range sometimes considered for the standard $\Lambda$CDM of $2\times10^{-8}$ becomes infeasible without ancillary low-frequency foreground information. An additional concern is dust absorption of the CMB monopole, a subtle effect that must be included. We quantify one form of model discrepancy error, finding that the error introduced by fitting our interstellar medium dust model with a modified blackbody is too large for CMB spectral distortions to be detectable. The greatest challenge may be the cosmic infrared background (CIB). We find that $\mu$ and $y$ are extremely sensitive to modeling choices for the CIB, and quantify biases expected for a range of assumptions.

==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/CIB_PC_variance.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
\footnotesize
\begin{tabular}{lrrrrrrrrrr}
\hline
PC Nr.   & 1       & 2       & 3       & 4       & 5       & 6       & 7        & 8        & 9        & 10       \\ \hline
PC Variance& 9.99e-01&6.16e-04&5.01e-05&1.51e-07&4.02e-09&1.59e-11&6.34e-12&1.56e-13&4.07e-14&4.95e-15 \\ \hline
\end{tabular}
\centering
\begin{tabular}{lrrrrrrrrrr}
\hline
PC Nr.   & 11       & 12       & 13       & 14       & 15       & 16       & 17        & 18        & 19        & 20       \\ \hline
PC Variance & 1.40e-15&1.50e-16&2.86e-17&3.11e-18&3.66e-19&4.39e-20&4.08e-21&4.63e-22&4.56e-23&4.41e-24 \\ \hline
\end{tabular}
\caption{The explained variance ratio of the first 20 principal components of the broadened CIB dataset. \label{table:CIB_PC_variance}}
\end{table*}

==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/ISM_dust_PC_fiducial.tex <==
\begin{table}[t]
\centering
\begin{tabular}{|r|r|r|r|r|r|}
\toprule
PC Parameter & WC0 & WC1 & WC2 & WC3  \\
\hline
Fiducial Value&8.3e+05&-2.4e+05&-3.6e+03&-6.7e+03 \\
\hline
\end{tabular}%
\caption{Fiducial values for the PCA coefficients used in the MCMC. The coefficients are obtained by decomposing a reference SED (shown in Fig. \ref{fig:foreground}) from the ISM dust posteriors from \cite{Zelko2020} unto the PCs. \label{table:PCA_initial}}
\end{table}

==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/ISM_dust_PC_variance.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
\footnotesize
\begin{tabular}{lrrrrrrrrrr}
\hline
PC Nr.   & 1       & 2       & 3       & 4       & 5       & 6       & 7        & 8        & 9        & 10       \\ \hline
Variance Ratio Fixed ISRF & 9.84e-01&1.59e-02&2.46e-04&4.15e-05&8.54e-07&2.11e-07&3.49e-08&1.97e-08&8.59e-09&2.09e-09 \\ \hline
Variance Ratio Variable ISRF & 9.75e-01&2.52e-02&2.59e-04&3.00e-05&3.66e-06&9.49e-07&2.62e-07&8.98e-08&2.42e-08&1.12e-08 \\ \hline
Var. Ratio Fixed ISRF No Shadow & 9.84e-01&1.59e-02&2.46e-04&4.16e-05&8.54e-07&2.12e-07&3.46e-08&1.97e-08&8.62e-09&2.05e-09 \\ \hline
Var. Ratio Variable ISRF No Shadow & 9.75e-01&2.52e-02&2.59e-04&3.00e-05&3.67e-06&9.55e-07&2.62e-07&8.97e-08&2.42e-08&1.11e-08 \\ \hline
\end{tabular}
\centering
\begin{tabular}{lrrrrrrrrrr}
\hline
PC Nr.   & 11       & 12       & 13       & 14       & 15       & 16       & 17        & 18        & 19        & 20       \\ \hline
Variance Ratio Fixed ISRF & 9.88e-10&2.07e-10&5.84e-11&4.36e-11&1.59e-11&8.68e-12&4.09e-12&1.64e-12&9.84e-13&5.84e-13 \\ \hline
Variance Ratio Variable ISRF & 1.99e-09&7.49e-10&3.27e-10&2.08e-10&4.72e-11&3.86e-11&1.54e-11&9.48e-12&6.81e-12&2.85e-12 \\ \hline
Var. Ratio Fixed ISRF No Shadow & 9.85e-10&2.06e-10&5.89e-11&4.38e-11&1.62e-11&8.65e-12&4.24e-12&1.65e-12&9.81e-13&5.84e-13 \\ \hline
Var. Ratio Variable ISRF No Shadow & 1.99e-09&7.48e-10&3.19e-10&2.05e-10&5.08e-11&3.92e-11&1.54e-11&9.50e-12&7.09e-12&2.84e-12 \\ \hline
\end{tabular}
\caption{The explained variance ratio of the first 20 principal components of the dust emissivity, for the cases of fixed and variable interstellar radiation field (ISRF). \label{table:ISM_dust_PC_variance}}
\end{table*}

==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/combos_table.tex <==
\begin{table*}[ht]
\setlength{\tabcolsep}{2.3pt}
\centering
\footnotesize
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
Param. &  $y \times 10^9$ & $\mu\times 10^9$& $\Delta_T$ &WC0&WC1&WC2&WC3&$ A_{\textnormal{s}}$ & $\alpha_{\textnormal{s}}$&$\omega_\textnormal{s}$ & $\alpha_{\textnormal{CIB}}$ & $\beta_{\textnormal{CIB}} $ & $T_{\textnormal{CIB}}$ & $A_{\textnormal{FF}}$  \\
\hline
Unit &  - & - & [nK] &  - &  - &  - &  - &[MJy/sr] &-& - & [MJy/sr] & - & [K] & [MJy/sr]  \\
\hline
Fid. & 1700&20&1.2e+05&8.3e+05&-2.4e+05&-3.6e+03&-6.7e+03&2.9e-04&-8.2e-01&2.0e-01&1.8e-03&8.6e-01&1.9e+01&3.0e-04 \\ \hline
$\sigma$ &0.9&9.8&1.7&1.0e+00&1.0e+00&1.0e+00&1.0e+00&-&-&-&-&-&-&- \\ \hline
$\sigma$ &1.5&23.9&5.4&-&-&-&-&3.0e-06&2.0e-03&6.5e-03&-&-&-&- \\ \hline
$\sigma$ &1.1&10.1&1.8&-&-&-&-&-&-&-&1.7e-08&6.6e-06&3.9e-05&- \\ \hline
$\sigma$ &1.0&11.5&2.3&-&-&-&-&-&-&-&-&-&-& 2.5e-07 \\ \hline
$\sigma$ &2.0&27.7&7.2&4.7e+00&2.1e+00&2.2e+00&1.5e+00&4.0e-06&9.9e-03&9.9e-03&-&-&-&- \\ \hline
$\sigma$ &1.5&10.8&2.6&7.6e+02&6.3e+01&1.1e+01&4.1e+00&-&-&-&2.9e-07&7.6e-05&2.4e-03&- \\ \hline
$\sigma$ &1.7&20.6&5.3&3.0e+00&1.5e+00&1.5e+00&1.2e+00&-&-&-&-&-&-& 8.3e-07 \\ \hline
$\sigma$ &2.2&33.9&11.1&-&-&-&-&7.3e-06&3.0e-02&2.7e-02&9.5e-08&2.9e-05&1.5e-04&- \\ \hline
$\sigma$ &1.7&34.1&8.6&-&-&-&-&3.8e-05&9.2e-02&5.6e-02&-&-&-& 1.3e-05 \\ \hline
$\sigma$ &1.5&20.7&5.3&-&-&-&-&-&-&-&2.5e-08&8.6e-06&4.9e-05& 9.2e-07 \\ \hline
$\sigma$ &7.4&140.5&58.8&8.8e+02&1.4e+02&2.7e+01&6.2e+00&4.5e-05&2.1e-01&1.9e-01&1.0e-06&4.1e-04&2.9e-03&- \\ \hline
$\sigma$ &3.1&62.9&17.3&5.3e+00&2.3e+00&2.4e+00&1.5e+00&8.2e-05&2.0e-01&1.2e-01&-&-&-& 2.9e-05 \\ \hline
$\sigma$ &2.0&22.0&6.0&7.6e+02&6.3e+01&1.1e+01&4.1e+00&-&-&-&2.9e-07&7.6e-05&2.4e-03& 9.5e-07 \\ \hline
$\sigma$ &2.3&44.6&12.9&-&-&-&-&6.7e-05&1.7e-01&1.1e-01&1.0e-07&3.1e-05&1.6e-04& 2.2e-05 \\ \hline
$\sigma$ &8.9&177.0&69.4&8.8e+02&1.4e+02&2.8e+01&6.6e+00&8.6e-05&2.6e-01&2.0e-01&1.1e-06&4.3e-04&3.0e-03& 3.1e-05 \\ \hline
\end{tabular}
\caption{Fisher information matrix estimates of uncertainty in $y$ and $\mu$ (full-sky average), allowing various combinations of foreground parameters to float (\S \ref{sec:fisherresults}).  In each row, the $1\sigma$ marginalized uncertainty is given for floating parameters, and fixed parameters are indicated by ``-''.  ISM dust is represented by 4 principal components, with emission spectra drawn from the \cite{Zelko2020} posterior (variable radiation field case).  Because the spectra are scaled by the PIXIE sensitivity in the PCA, the uncertainty of the PC coefficients (WCn) is 1.0 for the dust-only case, and larger for the other cases.  As more foreground parameters are allowed to float, the uncertainty in $y$ and $\mu$ grows.  When all foregrounds are included (bottom row), $\sigma_\mu$ is an order of magnitude larger than a case with fixed synchrotron parameters (3rd from bottom).  This suggests that independent constraints on the synchrotron spectrum would  substantially enhance the statistical power of PIXIE.  \label{table:combos_table}}
\end{table*}

==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/final_all_foregrounds_with_ISM_dust_4_PC_MCMC_results.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{1.5pt}
\centering
\scriptsize
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
Param Name & $y$&$\mu$&$\Delta_T$&WC0&WC1&WC2&WC3&$A_{\textrm{s}}$&$\alpha_{\textrm{s}}$&$\omega_{\textrm{s}}$&$A_{\textrm{FF}}$&$\alpha_{\textrm{CIB}}$&$\beta_{\textrm{CIB}}$&$T_{\textrm{CIB}}$ \\ \hline
Units & -&-&[K]&-&-&-&-&[MJy/sr]&-&-&[MJy/sr]&[MJy/sr]&-&[K] \\ \hline
Fiducial Val. & 1.70e-06&2.00e-08&1.20e-04&8.30e+05&-2.36e+05&-3.63e+03&-6.74e+03&2.88e-04&-8.20e-01&2.00e-01&3.00e-04&1.78e-03&8.60e-01&1.88e+01 \\ \hline
Post. Median & 1.70e-06&3.95e-08&1.20e-04&8.29e+05&-2.36e+05&-3.64e+03&-6.74e+03&2.77e-04&-8.03e-01&2.11e-01&3.07e-04&1.78e-03&8.60e-01&1.88e+01 \\ \hline
$\sigma_{+}$ & 8.41e-09&1.66e-07&6.37e-08&8.41e+02&1.22e+02&2.41e+01&6.48e+00&7.01e-05&1.34e-01&1.45e-01&2.97e-05&8.77e-07&3.74e-04&2.82e-03 \\ \hline
$\sigma_{-}$ & 8.33e-09&1.69e-07&6.37e-08&8.43e+02&1.14e+02&2.62e+01&6.29e+00&6.77e-05&2.48e-01&1.54e-01&3.35e-05&9.57e-07&3.46e-04&2.91e-03 \\ \hline
\end{tabular}
\caption{The results of the MCMC for the configuration checking the posterior is Gaussian for all foregrounds and 4 PC ISM dust. \label{table:foregrounds_MCMC}$ \sigma_{+}$ represents the difference between the 84th and 50th quantile of the posterior, and $\sigma{-}$ the one between the 50th and 16th.}
\end{table*}

==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/final_shadow_CIB_importance_ISM_dust_sync_free_MCMC_results.tex <==
\begin{table*}[ht]
\setlength{\tabcolsep}{1.5pt}
\centering
\footnotesize
\begin{tabular}{rrrrrrrrrrrrrr}
\hline
Param Name & $y$&$\mu$&$\Delta_T$&$\tau_{\textrm{D}}$&$\beta_{\textrm{D}}$&$T_{\textrm{D}}$&$A_{\textrm{s}}$&$\alpha_{\textrm{s}}$&$\omega_{\textrm{s}}$&$A_{\textrm{FF}}$&$\alpha_{\textrm{CIB}}$&$\beta_{\textrm{CIB}}$&$T_{\textrm{CIB}}$ \\ \hline
Units & -&-&[K]&-&-&[K]&[MJy/sr]&-&-&[MJy/sr]&[MJy/sr]&-&[K] \\ \hline
Fiducial Val. & 1.70e-06&2.00e-08&1.20e-04&2.32e-06&1.74e+00&1.82e+01&2.88e-04&-8.20e-01&2.00e-01&3.00e-04&1.78e-03&8.60e-01&1.88e+01 \\ \hline
Post. Median & 1.73e-06&-1.94e-07&1.19e-04&2.31e-06&1.74e+00&1.82e+01&2.52e-04&-9.00e-01&1.58e-01&3.13e-04&1.78e-03&8.62e-01&1.88e+01 \\ \hline
$\sigma_{+}$ & 4.57e-09&8.25e-08&2.90e-08&4.02e-09&1.26e-03&1.72e-03&3.97e-05&1.03e-01&7.07e-02&1.45e-05&3.39e-06&8.99e-04&2.66e-02 \\ \hline
$\sigma_{-}$ & 4.62e-09&8.11e-08&2.95e-08&4.12e-09&1.18e-03&1.90e-03&3.45e-05&1.17e-01&7.47e-02&1.61e-05&3.20e-06&8.71e-04&2.75e-02 \\ \hline
\end{tabular}
\caption{The results of the MCMC for the configuration testing the effect of not modeling the CIB shadow, with ISM dust, synchrotron and free-free foregrounds. \label{table:shadow_CIB}$ \sigma_{+}$ represents the difference between the 84th and 50th quantile of the posterior, and $\sigma{-}$ the one between the 50th and 16th. We observe that failing to include the CIB shadow results in a small bias in $y$ and a very large bias in $\mu$.}
\end{table*}

==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/final_shadow_ISM_dust_importance_sync_free_CIB_MCMC_results.tex <==
\begin{table*}[ht!]
\setlength{\tabcolsep}{1.5pt}
\centering
\footnotesize
\begin{tabular}{rrrrrrrrrrrrrr}
\hline
Param Name & $y$&$\mu$&$\Delta_T$&$\tau_{\textrm{D}}$&$\beta_{\textrm{D}}$&$T_{\textrm{D}}$&$A_{\textrm{s}}$&$\alpha_{\textrm{s}}$&$\omega_{\textrm{s}}$&$A_{\textrm{FF}}$&$\alpha_{\textrm{CIB}}$&$\beta_{\textrm{CIB}}$&$T_{\textrm{CIB}}$ \\ \hline
Units & -&-&[K]&-&-&[K]&[MJy/sr]&-&-&[MJy/sr]&[MJy/sr]&-&[K] \\ \hline
Fiducial Val. & 1.70e-06&2.00e-08&1.20e-04&2.32e-06&1.74e+00&1.82e+01&2.88e-04&-8.20e-01&2.00e-01&3.00e-04&1.78e-03&8.60e-01&1.88e+01 \\ \hline
Post. Median & 1.66e-06&-4.20e-07&1.20e-04&2.32e-06&1.74e+00&1.82e+01&3.61e-04&-6.62e-01&2.98e-01&2.64e-04&1.78e-03&8.59e-01&1.88e+01 \\ \hline
$\sigma_{+}$ & 5.91e-09&1.09e-07&3.95e-08&4.43e-09&1.42e-03&1.59e-03&8.02e-05&7.30e-02&3.73e-02&3.71e-05&3.66e-06&1.01e-03&2.86e-02 \\ \hline
$\sigma_{-}$ & 5.58e-09&1.18e-07&3.59e-08&4.63e-09&1.32e-03&1.81e-03&1.21e-04&3.15e-01&1.94e-01&3.54e-05&3.52e-06&9.66e-04&2.90e-02 \\ \hline
\end{tabular}
\caption{The results of the MCMC for the configuration testing the importance of modeling the ISM dust shadow, with CIB, synchrotron, and free-free foregrounds. \label{table:shadow_ISM}$ \sigma_{+}$ represents the difference between the 84th and 50th quantile of the posterior, and $\sigma{-}$ the one between the 50th and 16th. We observe that failing to include the ISM dust shadow results in a small bias in $y$ and a very large bias in $\mu$.}
\end{table*}

==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/fisher_ISM_dust_PC_results_table.tex <==
\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{1.1pt}
\begin{tabular*}{\linewidth}{ @{\extracolsep{\fill}}r *{10}{r} @{} }
\toprule
 & &\multicolumn{9}{c@{}}{Number of PCs used} \\
\cmidrule(l){3-11}
 & MBB & 2PC & 3PC & 4PC & 5PC & 6PC & 7PC & 8PC & 9PC & 10PC   \\
\midrule
\multicolumn{6}{@{}l@{}}{\textit{Fixed radiation field}} \\
$\sigma{y}$ &4.81e-09&5.85e-09 & 6.02e-09 & 6.02e-09 & 9.31e-09 & 9.33e-09 & 9.35e-09 & 1.02e-08 & 1.10e-08 & 1.23e-08 \\
$\sigma{\mu}$ &8.28e-08&1.11e-07 & 1.15e-07 & 1.16e-07 & 1.79e-07 & 1.81e-07 & 1.82e-07 & 1.96e-07 & 2.42e-07 & 2.72e-07 \\
\midrule
\multicolumn{6}{@{}l@{}}{\textit{Variable radiation field}} \\
$\sigma{y}$ &4.81e-09&4.41e-09 & 5.58e-09 & 8.89e-09 & 9.62e-09 & 1.18e-08 & 1.20e-08 & 1.30e-08 & 1.67e-08 & 1.78e-08 \\
$\sigma{\mu}$ &8.28e-08&8.36e-08 & 1.14e-07 & 1.77e-07 & 2.05e-07 & 2.63e-07 & 2.63e-07 & 2.83e-07 & 3.96e-07 & 4.09e-07 \\
\bottomrule
\end{tabular*}
\begin{tabular*}{\linewidth}{ @{\extracolsep{\fill}} r *{10}{r} @{} }
\toprule
 & &\multicolumn{9}{c@{}}{Number of PCs used} \\
\cmidrule(l){3-11}
 & 11PC & 12PC & 13PC & 14PC & 15PC & 16PC & 17PC & 18PC & 19PC & 20PC   \\
\midrule
\multicolumn{6}{@{}l@{}}{\textit{Fixed radiation field}} \\
$\sigma{y}$ &1.41e-08 & 1.46e-08 & 1.49e-08 & 2.15e-08 & 2.28e-08 & 2.44e-08 & 2.68e-08 & 2.77e-08 & 2.82e-08 & 2.86e-08 \\
$\sigma{\mu}$ &3.15e-07 & 3.32e-07 & 3.38e-07 & 5.36e-07 & 5.87e-07 & 6.14e-07 & 6.77e-07 & 7.20e-07 & 7.29e-07 & 7.44e-07 \\
\midrule
\multicolumn{6}{@{}l@{}}{\textit{Variable radiation field}} \\
$\sigma{y}$ &1.82e-08 & 1.86e-08 & 2.02e-08 & 2.48e-08 & 2.98e-08 & 3.54e-08 & 3.57e-08 & 3.57e-08 & 3.82e-08 & 3.91e-08 \\
$\sigma{\mu}$ &4.14e-07 & 4.30e-07 & 4.74e-07 & 5.94e-07 & 8.08e-07 & 9.40e-07 & 9.44e-07 & 9.45e-07 & 9.95e-07 & 1.02e-06 \\
\bottomrule
\end{tabular*}
\caption{Fisher Information Matrix analysis results. Standard deviations for the $y$ and $\mu$ parameters, given inclusion of various numbers of principal components. The case for constant and variable radiation field is shown. All other foregrounds are included in the analysis.  \label{table:results_table_1}}
\end{table*}


==> Proofed-Impact of Dust on CMB Spectral Distortions Measurements/parameters_fiducial.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{rrrrrrrrrrr}
\hline
Parameter Name  & $y$ & $\mu$& $\Delta_T$[K] & $ A_{\textnormal{s}}$[MJy/sr] & $\alpha_{\textnormal{s}} $&$\omega_\textnormal{s}$ & $\alpha_{\textnormal{CIB}}$[MJy/sr] & $\beta_{\textnormal{CIB}} $ & $T_{\textnormal{CIB}}$[K] & $A_{\textnormal{FF}}$[MJy/sr]\\ \hline
Fiducial Values & 1.7e-06&2.0e-08&1.2e-04&2.9e-04&-0.82&0.20&1.779e-03&0.86&18.80&3.0e-04 \\ \hline
\end{tabular}
\caption{The fiducial values of the spectral distortions and foreground parameters. The fiducial values for the ISM dust parameters are discussed in \S \ref{sec:dust_modeling} and \S \ref{sec:ISM_dust_forecasting_methods}. \label{table:foreground_fiducial_table}}
\end{table*}
